SD-LoRA: Scalable Decoupled Low-Rank Adaptation for Class Incremental Learning

Continual Learning (CL) with foundation models has recently emerged as a promising paradigm to exploit abundant knowledge acquired during pre-training for tackling sequential tasks. However, existing prompt-based and Low-Rank Adaptation-based (LoRA-based) methods often require expanding a prompt/LoRA pool or retaining samples of previous tasks, which poses significant scalability challenges as the number of tasks grows. To address these limitations, we propose Scalable Decoupled LoRA (SD-LoRA) for class incremental learning, which continually separates the learning of the magnitude and direction of LoRA components without rehearsal. Our empirical and theoretical analysis reveals that SD-LoRA tends to follow a low-loss trajectory and converges to an overlapping low-loss region for all learned tasks, resulting in an excellent stability-plasticity trade-off. Building upon these insights, we introduce two variants of SD-LoRA with further improved parameter efficiency. All parameters of SD-LoRAs can be end-to-end optimized for CL objectives. Meanwhile, they support efficient inference by allowing direct evaluation with the finally trained model, obviating the need for component selection. Extensive experiments across multiple CL benchmarks and foundation models consistently validate the effectiveness of SD-LoRA. The code is available at https://github.com/WuYichen-97/SD-Lora-CL.

==> Sec/1_intro.tex <==
\section{Introduction}
Continual Learning (CL)~\citep{rolnick2019experience,wang2024comprehensive,zhou2024class,wu2024meta} seeks to develop a learning system that can continually adapt to changing environments while retaining previously acquired knowledge. Unlike traditional supervised learning, which trains models on independent and identically distributed (i.i.d.) data, CL focuses on training models on non-stationary data distributions where tasks are presented sequentially. This deviation from the i.i.d assumption introduces the central challenge of mitigating catastrophic forgetting~\citep{french1999catastrophic, mcclelland1995there, mccloskey1989catastrophic,kirkpatrick2017overcoming}, a phenomenon characterized by a significant decline in performance on previously learned tasks.

% With the rise of large foundation models, researchers have found that these models not only facilitate effective knowledge transfer but also demonstrate improved resilience to catastrophic forgetting. Leveraging foundation models to address the forgetting issue has recently gained considerable attention. 

Over the last five years, large foundation models have demonstrated their effectiveness in enabling efficient knowledge transfer and showing greater resistance to catastrophic forgetting~\citep{wang2022learning,wang2022dualprompt,smith2023coda,wang2024hierarchical,wang2024hierarchical,liang2024inflora}. As a result, leveraging these foundation models to further mitigate forgetting have emerged as a key research area. One popular line of research involves manipulating the \textit{input and intermediate representations} (also referred to as the prompts) of foundation models.  L2P~\citep{wang2022learning} and DualPrompt~\citep{wang2022dualprompt} are pioneering methods that incrementally optimize a pool of prompts, which are selectively combined as the input in the model based on their distances to the incoming prompt, in a similar spirit to soft $K$-means clustering that does not rely on task index information. Coda-Prompt~\citep{smith2023coda} improves upon DualPrompt by end-to-end optimizing the prompt selection module. More recently, efforts to enhance performance have led to HidePrompt~\citep{wang2024hierarchical}, which not only employs incremental learning of prompts but also requires the storage of extensive sample features. \yichen{In a different approach,} InfLoRA~\citep{liang2024inflora} incrementally learns LoRA components instead of prompts, \yichen{yet it similarly necessitates the storage of large amounts of sample features.}
% Although InfLoRA~\citep{liang2024inflora} takes a different approach by incrementally learning LoRA components instead of prompts, it shares the need for storing large amounts of sample features. 

As shown in Table~\ref{tab:related_work}, current CL methods \yichen{leveraging} foundation models \yichen{typically} necessitate the incremental storage of structures and often rely on 
extensive sample feature storage. However, as the number of sequential tasks increases, the continual expansion of prompts or LoRA components, along with the growing storage costs of sample features, becomes inefficient and unsustainable. This leads to two key challenges for CL with foundation models: (1) \yichen{the relationship between the incrementally added structures remains unexplored, making it unclear when further expansion is unnecessary;} and (2) \yichen{how can we improve the efficiency of CL while maintaining strong performance, particularly by reducing the need for continually adding new structures (i.e., LoRA, prompts) and minimizing reliance on sample feature storage?}

% there is a lack of exploration into the relationship between the incrementally added structures, leaving it unclear under what conditions further expansion is unnecessary; (2) how can we maximize the efficiency of CL while maintaining its average performance, particularly by reducing the need for continually adding structures (i.e., LoRA, prompts) and eliminating the reliance on sample feature storage?

% \begin{itemize}[leftmargin=10mm, itemsep=-1mm, topsep=-0.5 mm]
%     \item[$\circ$] There is a lack of exploration into the relationship between the incrementally added structures, leaving it unclear under what conditions further expansion is unnecessary.
%     \item[$\circ$] How can we maximize the efficiency of CL while maintaining its average performance, particularly by reducing the need for continually adding structures (i.e., LoRA, prompts) and eliminating the reliance on sample feature storage?
% \end{itemize}
% However, as the number of streaming tasks increases, consistently continually augmenting prompts or LoRA components becomes inefficient and unsustainable.
% As shown in Table XXX, current CL with foundation models require storing the structures in an incrementally way, and even need to store extensive sample features. As the number of streaming tasks grows, continually increasing prompts or LoRA components becomes inefficient and unsustainable.
% More recently, in an effort to further improve performance, HidePrompt not only requires incremental learning of the prompts but also needs to store extensive sample features. InfLoRA is similar to HidePrompt while it incrementally learn the LoRA part instead of the prompt. However, with the growing number of streaming tasks, continually increasing prompts or LoRA components becomes inefficient and xxx.
% Consequently, the exploration of strategies to leverage foundation models for mitigating the forgetting issue has recently garnered significant attention.  For instance, L2P~\cite{wang2022learning} and DualPrompt are the first to create a pool of prompts to be selected for insertion into the model, matching input data to prompts without task index with a local clustering-like optimization.  Coda-Prompt assembles learnable prompt components which are then inserted into a pre-trained ViT encoder for image classification with an end-to-end fashion.
% To address these challenges, we first attempt a Simple yet Effective algorithm, SE-LoRA, which integrates a low-rank adaptation module and incrementally adds LoRA components while decoupling the learning of direction and magnitude. This approach allows for a more thorough exploration of the interrelationship between these factors. Surprisingly, we found this simple method to be highly effective, achieving excellent performance. 
\begin{table}[t]
\centering
% \caption{Summary of existing CL methods utilizing foundation models. }
\caption{\yichen{Comparisons of existing CL methods with foundation models.  \textit{Store Samples/Features} indicates whether a method requires storing features from previously trained samples to enhance performance. \textit{Store Structures/Weights} shows if additional modules are needed to fine-tune the foundation model. \textit{Incrementally Expand} refers to whether the method endlessly adds new components—such as LoRA, prompts, or sample features—after training each new task. }}
\label{tab:related_work}
 	% \setlength{\tabcolsep}{0.3 mm}{
    \resizebox{130mm}{13mm}{
 	    \begin{tabular}{c|c|c|c} 
			\toprule
			\multicolumn{1}{l}{\multirow{2}{*}{\textbf{Method}}} &
			\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Incrementally Expand}}} & 
			\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Store Samples/Features}}} & 
			\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Store Structures/Weights}}}  \\
			\multicolumn{1}{l}{\multirow{2}{*}{}} &
			\multicolumn{1}{c}{\multirow{2}{*}{}} & 
			\multicolumn{1}{l}{\multirow{2}{*}{}} &
			\multicolumn{1}{c}{\multirow{2}{*}{}} \\
			\midrule
			\multicolumn{1}{l}{\multirow{1}{*}{L2P~\citep{wang2022learning}}} &
			\multicolumn{1}{c}{\multirow{1}{*}{\ding{51}}} & 
			\multicolumn{1}{c}{\multirow{1}{*}{\ding{55}}} &
			\multicolumn{1}{c}{\multirow{1}{*}{\ding{51}}} \\
			
			\multicolumn{1}{l}{\multirow{1}{*}{DualPrompt~\citep{wang2022dualprompt}}} &
			\multicolumn{1}{c}{\multirow{1}{*}{\ding{51}}} & 
			\multicolumn{1}{c}{\multirow{1}{*}{\ding{55}}} &
			\multicolumn{1}{c}{\multirow{1}{*}{\ding{51}}} \\

			\multicolumn{1}{l}{\multirow{1}{*}{HidePrompt~\citep{wang2024hierarchical}}} &
			\multicolumn{1}{c}{\multirow{1}{*}{\ding{51}}} & 
			\multicolumn{1}{c}{\multirow{1}{*}{\ding{51}}} &
			\multicolumn{1}{c}{\multirow{1}{*}{\ding{51}}} \\
            
			\multicolumn{1}{l}{\multirow{1}{*}{InfLoRA~\citep{liang2024inflora}}} &
			\multicolumn{1}{c}{\multirow{1}{*}{\ding{51}}} & 
			\multicolumn{1}{c}{\multirow{1}{*}{\ding{51}}} &
			\multicolumn{1}{c}{\multirow{1}{*}{\ding{51}}} \\

			\multicolumn{1}{l}{\multirow{1}{*}{ES-LoRA(Ours)}} &
			\multicolumn{1}{c}{\multirow{1}{*}{\ding{55}}} & 
			\multicolumn{1}{c}{\multirow{1}{*}{\ding{55}}} &
			\multicolumn{1}{c}{\multirow{1}{*}{\ding{51}}} \\			
			\bottomrule
		\end{tabular}
  
		}
\vspace{-3mm}
\end{table}

To address these challenges, \yichen{we propose a simple and scalable algorithm based on low-rank adaptation, S-LoRA, which incrementally adds LoRA components while decoupling the learning of its direction and magnitude. This allows for a more thorough examination of the interrelationships among the incrementally added LoRA parts. Interestingly, S-LoRA demonstrates exceptional effectiveness and achieves high performance. To further understand the underlying mechanisms of S-LoRA, we conduct an in-depth analysis and find that its success stems from learning a low-loss path that converges to a shared low-loss region.  Moreover, the importance of its incrementally learned directions (i.e., LoRA) gradually decreases during sequential training. This insight inspires us to develop more efficient versions, ES-LoRA, which alleviate or even eliminate the issue of continuous expansion without the need for additional feature storage. In summary, our contributions are as follows:} 
% To address these challenges, we first attempt a Simple yet Effective algorithm, SE-LoRA, which integrates a low-rank adaptation module and incrementally adds LoRA components while decoupling the learning of direction and magnitude. This approach allows for a more thorough exploration of the interrelationship between these factors. Surprisingly, we found this simple method to be highly effective, achieving excellent performance. To further investigate the underlying mechanisms of SE-LoRA, we conduct a comprehensive analysis and discover that its success derives from learning a low-loss path that converges to a shared low-loss region. Moreover, the importance of its incrementally learned directions (i.e., LoRA) gradually decreases during the sequential training. This inspires us to design several more efficient versions of SE-LoRA, which can alleviate or even eliminate the problem of incremental expansion without storing additional sample features. In summary, our contributions are as follows: 

\begin{itemize}[leftmargin=4mm, itemsep=0mm, topsep=-0.5 mm]
    \item[$\circ$] \yichen{We introduce S-LoRA, a method that decouples the learning of direction and magnitude, allowing us to examine the interrelationships among the added components more effectively.}
    % We first propose the S-LoRA, which incrementally decouples the learning of direction and magnitude and enables us to explore the interrelationship among the incrementally added components.
    % We propose SE-LoRA, an effective method that decouples the learning of direction and magnitude to enhance efficiency in class incremental learning.
    \item[$\circ$] \yichen{We conduct both theoretical and experimental analyses to investigate the effectiveness of S-LoRA, discovering that the significance of the learned LoRA diminishes during sequential training.}
    % We provide the theoretical and experimental analysis to explore the reason why it is effectiveness of the proposed S-LoRA. And found that the importance of the incrementally learned directions (i.e., LoRA) gradually decreases during sequential training.
    
    \item[$\circ$] \yichen{Based on our findings, we develop efficient versions of S-LoRA, termed ES-LoRA, which reduce the need for continuous expansion and eliminate the requirement for additional feature storage.}
    % Building on the analysis, we develop more efficient versions of S-LoRA, ES-LoRA, which reduces the need for continual expansion and eliminating additional sample feature storage.
    \item[$\circ$] \yichen{We validate the strong performance of S-LoRA and ES-LoRA through comprehensive experiments across multiple class incremental learning scenarios and backbones.}
    % We conduct extensive experiments validating the superior performance of SE-LoRA in various class incremental learning scenarios.
\end{itemize}



% (1) we propose SE-LoRA, an effective method that decouples the learning of direction and magnitude to enhance efficiency in class incremental learning; (2) we provide a theoretical and experimental analysis of the SE-LoRA mechanism, demonstrating that early learned directions play a crucial role in minimizing loss across sequential tasks; (3) we develop more efficient versions of SE-LoRA, reducing the need for continual expansion and eliminating additional sample feature storage; (4) we conduct extensive experiments validating the superior performance of SE-LoRA in various class incremental learning scenarios.

% To address these challenges, in this paper, we first attempt to propose the SE-LRA algorithm, which adopts the low-rank adaptation module and incrementally decouples the learning of direction and magnitude. By exploring the effective mechanism of 



% With the development of the large foundation models, it has been validated that they can not only significantly deliver knowledge transfer but also enhance resilience to catastrophic forgetting. How to utilize the foundation model to alleviate the forgetting problem has recently become a hot topic in this area. For instance, L2P XXXX, DualPrompt.

% With the development of the large foundation model, more works has try to 


% Due to the violation of the i.i.d assumption, the central challenge in continual learning is to mitigate catastrophic forgetting [\textbf{CITE}], a phenomenon where there is a significant drop in performance on previously learned tasks.

% Continual Learning (CL) hopes to construct a learning system that can continuously adapt to changing environments while retaining previously learned knowledge. Different from traditional supervised learning, which trains models on independent and identically distributed (i.i.d) data, CL aims to train a model on non-stationary data distributions where different tasks are presented sequentially. The primary problem in the CL area is to alleviate the catastrophic forgetting problem where there is a significant performance drop in testing performance on previously learned tasks.

%Specifically,  Continual Learning hopes the models are designed to sequentially acquire and adapt to new tasks over time while retaining previously learned knowledge. 

==> Sec/2-related-submit.tex <==
\section{Related Work} 
\textbf{Continual Learning (CL).} CL seeks to sequentially learn from new tasks while retaining previously acquired knowledge, with the central goal of mitigating catastrophic forgetting. Broadly, existing CL methods can be categorized according to three main design philosophies: Rehearsal-based, regularization-based, and architecture-based approaches. Rehearsal-based methods~\citep{riemer2018learning,chaudhry2019tiny, wang2023cba, wang2024dual,wu2024mitigating} selectively retain and replay samples from previous tasks to alleviate catastrophic forgetting. Regularization-based methods~\citep{kirkpatrick2017overcoming, li2017learning, lee2019overcoming, wu2024meta} introduce penalty terms into the training objective to constrain updates on parameters deemed important for learned tasks. Architecture-based methods~\citep{mallya2018piggyback, ebrahimi2020adversarial, ramesh2021model} expand or adapt the model architecture to account for new tasks. By allocating additional task-specific parameters or modules, these methods prevent the overwriting of learned important weights. Among various CL settings, this paper focuses on particularly challenging and practical class-incremental learning, in which the model must perform all learned tasks with no access to task identity at test time. Conventional class-incremental learning methods often require expensive training from scratch or parameter-intensive tuning, which can lead to overfitting and interference among tasks.


\textbf{CL with Foundation Models.} Foundation models have recently demonstrated their effectiveness in CL by facilitating knowledge transfer across tasks and reducing catastrophic forgetting~\citep{wang2022learning,wang2022dualprompt,smith2023coda,wang2024hierarchical,liang2024inflora, piao2024federated, zhiqi2025advancing}. Specifically, 
methods like L2P~\citep{wang2022learning}, DualPrompt~\citep{wang2022dualprompt}, and CODA-Prompt~\citep{smith2023coda} integrate Vision Transformers (ViTs) with prompt-tuning strategies~\citep{lester2021power,jia2022visual}, thereby improving knowledge retention as new tasks are introduced. Building on these, HiDe-Prompt~\citep{wang2024hierarchical} further stores a large number of samples to boost performance. Rather than prompt-tuning, InfLoRA~\citep{liang2024inflora} adopts a LoRA-based Parameter-Efficient Fine-Tuning (PEFT) approach, which similarly necessitates substantial sample storage. Despite their promise, none of the existing CL methods with foundation models simultaneously satisfy the three desirable properties outlined in Table~\ref{tab:related_work}. To fill this gap, we introduce SD-LoRA, which can also be viewed as a form of model-merging techniques~\citep{chitale2023task,ilharco2023editing}, developed in parallel with, yet complementary to ongoing CL research.

\textbf{Parameter-Efficient Fine-Tuning (PEFT).} The integration of PEFT methods with CL with foundation models is essential because full fine-tuning for each individual task is prohibitive in terms of computation and storage requirements. Representative PEFT methods include {adapters}~\citep{houlsby2019parameter}, which insert lightweight learnable modules into Transformer layers;  {prompt-tuning}~\citep{qin2021learning,jia2022visual} and {prefix-tuning}~\citep{li2021prefix}, which introduce learnable input representations into Transformer layers; and  {LoRA}~\citep{hulora2022}, which adds and tunes low-rank branches as updates to the pre-trained weights. While these techniques have proven effective in single-task and multi-task offline learning settings, their performance boundaries in CL with foundation models remain insufficiently explored. The proposed SD-LoRA adopts a rehearsal-free, LoRA-based PEFT approach for CL with foundation models.
